Robotic Monitoring of Colorimetric Leaf Sensors for Precision Agriculture

Common remote sensing modalities (RGB, multispectral, hyperspectral imaging or LiDAR) are often used to indirectly measure crop health and do not directly capture plant stress indicators. Commercially available direct leaf sensors are bulky, powered electronics that are expensive and interfere with crop growth. In contrast, low-cost, passive and bio-degradable leaf sensors offer an opportunity to advance real-time monitoring as they directly interface with the crop surface while not interfering with crop growth. To this end, we co-design a sensor-detector system, where the sensor is a passive colorimetric leaf sensor that directly measures crop health in a precision agriculture setting, and the detector autonomously obtains optical signals from these leaf sensors. The detector comprises a low size weight and power (SWaP) mobile ground robot with an onboard monocular RGB camera and object detector to localize each leaf sensor, as well as a hyperspectral camera with a motorized mirror and halogen light to acquire hyperspectral images. The sensor's crop health-dependent optical signals can be extracted from the hyperspectral images. The proof-of-concept system is demonstrated in row-crop environments both indoors and outdoors where it is able to autonomously navigate, locate and obtain a hyperspectral image of all leaf sensors present, and acquire interpretable spectral resonance with 80 $\%$ accuracy within a required retrieval distance from the sensor.

==> notes.tex <==
\begin{enumerate}
    \item Questions: next best view or visual servoing?
    \item TODO: plugging in dongle to beast; set the master to beast, not 
    \item lux meter
    \item Any data/figure that drives home the fact that we have a complicated system. Venn diagram/table with ticks with systems with individual components, and our system ticks all of the boxes. 
    \item each sub-system should be state of the art / novel. new=spectralzoom; leaf sensor; robot with yolo + sensor suite.
    \item lux measurements.
    \item wouldn't the person deploying the sensors then be able to report back on which plants the sensors are placed? Having this unknown seems unrealistic?
    \item can we travel in a straight line. If it is raining, we should test this indoors.
    \item pavement might not be sellable, we might need to travel over grass/mud
    \item if we still cannot go over grass and to make this possible would take time, consider putting the orange component (hyperspectral+rgb) on top of the Jackal?
    \item for Shobhita: looking for leaf sensor novelty, and comparison to leaf sensors used in an ag setting/published lit on leaf sensors 
    \item if we want more claimed contributions, can consider estimating the angle of the sensor (if we know a certain angle gives a more optimal/informative spectra), obtain the affine transformations between the corners of the skew sensor and the non-skew/normal sensor
    \item if we want more claimed contributions, the homography from RGB to hyperspectral (via the mirror), summarize what we did to get this, and check if Jackson's past papers already did this 
    \item we need better arguments for why we have a new robot, and are not using the jackal

\end{enumerate}



%Indoors $\rightarrow$ outdoors?
% \section{Planner}
% \begin{enumerate}
%     \item Pipeline diagram with the task/behavior planner
%     \item High level topological/grid cell map, online lower level metric/semantic map? Pre-planning with incomplete information (only traversable region but at early stage of growth, i.e., not conservative) and reactive planning for obstacle avoidance (not navigating into the crops) based on partially known environment and online refinement of robot pose during mission (according for robot vehicle config/kinematics) for information gathering of ROI. Specific maneuver/behavior is required based on incoming observations.
%     \item MAYBE. Assume that there exists spatial correlations amongst observations for ROI, and plan adaptively (not every leaf sensor needs to be read?). Maybe we can do this in simulation?
%     \item map/information representation/gathering, localization, planning, reactive control 
%     \item remember that navigation/maneuverability/locomotion is directly tied to the task.
%     \item robust to different levels of environment, e.g., dense foliage, less dense foliage, lighting conditions 
% \end{enumerate}

% Incorporate additional behavior: Take multiple images.

% Continual behavior: Obstacle avoidance  %(https://github.com/tiralonghipol/t265_depth)

==> text/robot_state_estimation.tex <==
% \subsection{Navigation $\rightarrow$ Robot State Estimation \Alice{Malakhi}}\label{sec:ukf}
%RC navigation $\rightarrow$ obstacle avoidance navigation?
%To traverse its environment autonomously, the \textsc{beast} robot utilizes a RealsenseT265 for Visual-Inertial-Odometry which provides uncertain real-time data, and a SparkFun Real-Time-Kinematic Global Positioning System which provides certain but infrequent data.
%Relying on a pre-existing obstacle and target map, the robot employs RRT* navigation to adeptly maneuvers around obstacles en route to its destination.
%the target plant, the robot diligently scans the vicinity to locate a sensor. 
% In executing its autonomous navigation tasks, the \textsc{beast} robot integrates sophisticated sensor technologies to navigate its surroundings effectively. Leveraging the Realsense T265 for Visual-Inertial-Odometry, the robot acquires real-time data, albeit with inherent uncertainties, crucial for assessing its dynamic environment. Additionally, the incorporation of the SparkFun Real-Time-Kinematic Global Positioning System furnishes the robot with intermittently received but highly accurate positional data, offering crucial guidance amidst uncertain terrain.

% To successfully complete its navigation strategy, apriori obstacle and target maps are utilized. The robot uses an Ackerman Steering controller that delivers linear and angular velocity commands based on odometry input. The robot employs a Rapidly-exploring Random Trees Star (RRT*) navigation algorithm, allowing it to adeptly navigate cluttered environments while circumventing obstacles. This tree is pruned to only allow nodes that fall within the robots estimated turning radius, which is augmented from the normal bicycle-model because of the robot's front and rear steering and drive.



==> text/system_overview.tex <==
% In this letter, we use the ground robot platform described in Sec. \ref{sec:robot_platform} to demonstrate the proposed next best pose planning pipeline illustrated in Fig. \ref{fig:pipeline} for novel leaf sensor detection and hyperspetral reflectance imaging.
% Each sub-component of the system is described in their respective sections.
% To extract information from a colorimetric leaf sensor detailed in Sec. \ref{sec:leaf_sensor}, an object detector described in Sec. \ref{sec:yolo} is trained to detect the leaf sensor from incoming RGB images.
% A filter in Sec. \ref{sec:visual_servoing} is used to maintain a belief of the position of the leaf sensor and a planner is to select the next best pose of the robot to acquire a hyperspectral reflectance image of the leaf sensor.
% Based on unscented Kalman filter (UKF) robot state estimates, the robot updates its pose to reduce the error between its current and desired robot pose for hyperspectral image acquisition.
% When the desired pose is reached, the hyperspectral camera described in Sec. \ref{sec:hyperspectral} acquires a hyperspectral reflectance image of the leaf sensor in the scene.

% detect and track a colorimetric leaf sensor detailed in Section \ref{sec:leaf_sensor}, where detection is described in Section \ref{sec:yolo}. To perform this task, the robot navigates in the environment using a UKF described in \ref{sec:ukf}. 
% % \VM{Maybe also consider making a pipeline diagram.}
% % \textcolor{blue}{Make pipeline diagram}


%{Ideally this is like a full width figure.}



==> text/visual_servoing.tex <==
\VM{Unclear what the planning problem here is?}
% Robot odometry is estimated using Stereolabs Terra AI's Zed X.
% Given the focal length of the hyperspectral camera, known physical size of the leaf sensor and YOLO bounding box location and size, the robot repositions itself to reach a pose suitable for acquiring a hyperspectral image.
% such that the bounding box of the leaf sensor from YOLO is of a.

% Based on thorough in-lab laboratory-grade spectrometer and outdoor hyperspectral experimentation, we determined that the most informative hyperspectral signatures, associated with high signal-to-noise ratio, are obtained when light rays reflected from the surface of the leaf sensor are at a $45^\circ$ incidence angle to the hyperspectral mirror surface \textcolor{blue}{Shobhita, can you check this phrasing}.

% Collectively, this definition of the most informative pose of the robot relative to the leaf sensor, the extrinsics of the hyperspectral camera and mirror on the robot, and the robot's current belief of the leaf sensor are all used to determine the next best pose of the robot. 
% The robot performs visual servoing to update its pose, reducing the error between its current and most informative pose.

% We find the pixel co-ordinates of the leaf sensor in the camera frame $\mathcal{U}^{RGB}$, and estimate the world 3D co-ordinate of the sensor assuming that we know the size of the sensor.
% Once the sensor, has been detected we rotate the gimbal of the camera such that the sensor is centered in the camera frame of the robot.

% TODO: include Bayes filter/log-updates of the yolo observations, and `move forward as the uncertainty decreases, and move back once it starts to increase'.
